HSVI for zs-POSGs using Concavity, Convexity and Lipschitz Properties

Dynamic programming and heuristic search are at the core of state-of-the-art solvers for sequential decision-making problems. In partially observable or collaborative settings (\eg, POMDPs and Dec-POMDPs), this requires introducing an appropriate statistic that induces a fully observable problem as well as bounding (convex) approximators of the optimal value function. This approach has succeeded in some subclasses of 2-player zero-sum partially observable stochastic games (zs-POSGs) as well, but failed in the general case despite known concavity and convexity properties, which only led to heuristic algorithms with poor convergence guarantees. We overcome this issue, leveraging on these properties to derive bounding approximators and efficient update and selection operators, before deriving a prototypical solver inspired by HSVI that provably converges to an $\epsilon$-optimal solution in finite time, and which we empirically evaluate. This opens the door to a novel family of promising approaches complementing those relying on linear programming or iterative methods.

==> Makefile <==
DEPS_DIR = .deps
LATEXMK = latexmk -recorder -use-make -deps \
	-e 'warn qq(In Makefile, turn off custom dependencies);' \
	-e '@cus_dep_list = ();' \
	-e 'show_cus_dep();'

extended.pdf : extended.tex Makefile
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	-$(LATEXMK) -pdf -deps-out=$(DEPS_DIR)/$@P $<
	./clean-deps.sh $(DEPS_DIR)/$@P

clean :
	rm -f *~
	latexmk -c

veryclean:
	rm -rf *~ .deps *.bbl figures/*.bak
	latexmk -C


==> figures/dag.tex <==
\def\sScript{.7} % useless if =1
\def\sTiny{0.1} % currently unused

% \newcommand{\nodeW}[3]{$(\occ,\nu,\delta,\beta_{#3})_{#2}^{#1}$}
% \newcommand{\nodeW}[2]{
%   $\substack{
%     \langle \occ^{c,1}_{\depth-1}, \beta^2_{\depth-1}, \quad \\ %
%     \langle \delta^2_\depth, \upb\nu^2_\depth \rangle
%     \rangle_{#2}^{#1}
%   }$
% }
\newcommand{\nodeW}[2]{
  $\begin{array}{@{}c@{}c@{}l@{}}
     \langle
     & \occ^{c,1}_{\depth-1}, \beta^2_{\depth-1}
     &,  \\ %
     & \langle \delta^2_\depth, \upb\nu^2_\depth \rangle
     & \rangle_{#2}^{#1}
   \end{array}
   $
}
\newcommand{\nodeWLast}[2]{
  $\begin{array}{@{}c@{}c@{}l@{}}
     \langle
     & \occ^{c,1}_{\depth-1}, \beta^2_{\depth-1}
     &,  \\ %
     & -
     & \rangle_{#2}^{#1}
   \end{array}
   $
}

\colorlet{lightgray}{gray!35}

\begin{tikzpicture}

  \def\radA{1cm} % {.6cm}
  \def\radB{4cm} % {3cm}
  \def\radC{7.5cm}
  \def\myshape{rectangle} % circle/ellipse/rectangle/...
  
  % 0th line: root node only
  \node [ellipse, draw, scale=1] (n0) at (0,0) {$\langle \occ^{c,1}_\depth, \delta^2_\depth, \upb\nu^2_\depth \rangle_0$};
  \node [scale=\sScript] at (\radC,0) {$\depth=0$};
  
  % 1st line
  \node [below = 1cm of n0] (n1dots) { $\cdots$ };
  \node [\myshape, draw, scale=\sScript, left = \radB of n1dots] (n11) { \nodeW{1}{1} };
  \node [\myshape, draw, scale=\sScript, left = \radA of n1dots] (n12) { \nodeW{2}{1} };
  \node [\myshape, draw, scale=\sScript, right = \radB of n1dots] (n1n) { \nodeW{n_1}{1} };
  \node [\myshape, draw, scale=\sScript, right = \radA of n1dots] (n1n1) { \nodeW{n_1-1}{1} };
  % \node [right = 5cm of n1dots] {$\depth=1$};
  %\node at (6,-2) {$\depth=1$};
  \node [below = 1cm of n0, xshift=\radC, scale=\sScript] {$\depth=1$};
  
  \draw[->] (n0) -- (n11);
  \draw[->] (n0) -- (n12);
  \draw[->] (n0) -- (n1n);
  \draw[->] (n0) -- (n1n1);
  
  % 2nd line
  \node [below = 2cm of n1dots] (n2dots) { $\cdots$ };
  %\node at (0,-5) (n2dots) { $\cdots$ };
  \node [\myshape, draw, scale=\sScript, left = \radB of n2dots] (n21) { \nodeW{1}{2} };
  \node [\myshape, draw, scale=\sScript, left = \radA of n2dots] (n22) { \nodeW{2}{2} };
  \node [\myshape, draw, scale=\sScript, right = \radB of n2dots] (n2n) { \nodeW{n_2}{2} };
  \node [\myshape, draw, scale=\sScript, right = \radA of n2dots] (n2n1) { \nodeW{n_2-1}{2} };
  %\node [right = 5cm of n2dots] {$\depth=2$};
  %\node at (6,-5) {$\depth=2$};
  \node [below = 2cm of n1dots, xshift=\radC, scale=\sScript] {$\depth=2$};
  
  \draw[->, lightgray] (n12) -- (n21);
  %\draw[->, lightgray] (n12) -- (n22);
  \draw[->, lightgray] (n12) -- (n2n1);
  %\draw[->, lightgray] (n12) -- (n2n);
    
  \draw[->, lightgray] (n1n1) -- (n21);
  %\draw[->, lightgray] (n1n1) -- (n22);
  \draw[->, lightgray] (n1n1) -- (n2n);
  %\draw[->, lightgray] (n1n1) -- (n2n1);
  
  %\draw[->, lightgray] (n1n) -- (n21);
  \draw[->, lightgray] (n1n) -- (n22);
  \draw[->, lightgray] (n1n) -- (n2n);
  \draw[->, lightgray] (n1n) -- (n2n1);
  
  \draw[->] (n11) -- (n21);
  \draw[->] (n11) -- (n22);
  \draw[->] (n11) -- (n2n1);
  %\draw[->] (n11) -- (n2n);

  \node [below of = n21] (n21vdots) { $\vdots$ };
  \node [below of = n2dots] (n2dotsvdots) { $\vdots$ };
  \node [below of = n2n] (n2nvdots) { $\vdots$ };
  \node [below of = n2dots, xshift=\radC, scale=\sScript] {$\vdots$};
  
  % H-1 th line
  \node [below = .7cm of n2dotsvdots] (nH2dots) { $\cdots$ };
  \node [\myshape, draw, scale=\sScript, left = \radB of nH2dots] (nH21) { \nodeW{1}{H-2} };
  \node [\myshape, draw, scale=\sScript, left = \radA of nH2dots] (nH22) { \nodeW{2}{H-2} };
  \node [\myshape, draw, scale=\sScript, right = \radB of nH2dots] (nH2n) { \nodeW{n_{H-2}}{H-2} };
  \node [\myshape, draw, scale=\sScript, right = \radA of nH2dots] (nH2n1) { \nodeW{n_{H-2}-1}{H-1} };
  % \node [right = 5cm of nH2dots] {$\depth=H-2$};
  \node [below = .7cm of n2dotsvdots, xshift=\radC, scale=\sScript] {$\depth=H-2$};
  
  % Hth line
  \node [below = 2cm of nH2dots] (nH1dots) { $\cdots$ };
  \node [\myshape, draw, scale=\sScript, left = \radB of nH1dots] (nH11) { \nodeWLast{1}{H-1} };
  \node [\myshape, draw, scale=\sScript, left = \radA of nH1dots] (nH12) { \nodeWLast{2}{H-1} };
  \node [\myshape, draw, scale=\sScript, right = \radB of nH1dots] (nH1n) { \nodeWLast{n_{H-1}}{H-1} };
  \node [\myshape, draw, scale=\sScript, right = \radA of nH1dots] (nH1n1) { \nodeWLast{n_{H-1}-1}{H-1} };
  % \node [right = 5cm of nH1dots] {$\depth=H-1$};
  \node [below = 2cm of nH2dots, xshift=\radC, scale=\sScript] {$\depth=H-1$};
  
  %\draw[->, lightgray] (nH22) -- (nH11);
  \draw[->, lightgray] (nH22) -- (nH12);
  \draw[->, lightgray] (nH22) -- (nH1n1);
  %\draw[->, lightgray] (nH22) -- (nH1n);
    
  \draw[->, lightgray] (nH2n1) -- (nH11);
  %\draw[->, lightgray] (nH2n1) -- (nH12);
  \draw[->, lightgray] (nH2n1) -- (nH1n);
  %\draw[->, lightgray] (nH2n1) -- (nH1n1);
  
  %\draw[->, lightgray] (nH2n) -- (nH11);
  \draw[->, lightgray] (nH2n) -- (nH12);
  %\draw[->, lightgray] (nH2n) -- (nH1n);
  \draw[->, lightgray] (nH2n) -- (nH1n1);
  
  \draw[->] (nH21) -- (nH11);
  %\draw[->] (nH21) -- (nH12);
  \draw[->] (nH21) -- (nH1n1);
  %\draw[->] (nH21) -- (nH1n);
  
\end{tikzpicture}

